"What Are You Trying to Do?" Semantic Typing of Event Processes

This paper studies a new cognitively motivated semantic typing task, multi-axis event process typing, that, given an event process, attempts to infer free-form type labels describing (i) the type of action made by the process and (ii) the type of object the process seeks to affect. This task is inspired by computational and cognitive studies of event understanding, which suggest that understanding processes of events is often directed by recognizing the goals, plans or intentions of the protagonist(s). We develop a large dataset containing over 60k event processes, featuring ultra fine-grained typing on both the action and object type axes with very large ($10^3\sim 10^4$) label vocabularies. We then propose a hybrid learning framework, P2GT, which addresses the challenging typing problem with indirect supervision from glosses1and a joint learning-to-rank framework. As our experiments indicate, P2GT supports identifying the intent of processes, as well as the fine semantic type of the affected object. It also demonstrates the capability of handling few-shot cases, and strong generalizability on out-of-domain event processes.

==> tables/processes.tex <==
\begin{table}[!t]
    \centering
    %\resizebox{\columnwidth}{!}
    \setlength{\tabcolsep}{3pt}
    {%
    \small
    \begin{tabular}{p{0.66\linewidth}|p{0.27\linewidth}}
    \hline
    \toprule
     \textbf{Event processes} & \textbf{Types} \\ 
     \hline
     \multirow{2}{1.\linewidth}{Dig a hole $\Rightarrow$ Put seeds $\Rightarrow$ Fill soil $\Rightarrow$ Water soil} & \textbf{Action:}\emph{Plant}\\
     & \textbf{Object:}\emph{Plant}\\
     \hline
     \multirow{2}{1.\linewidth}{Fill a highball with ice $\Rightarrow$ Add vodka $\Rightarrow$ Add pineapple juice $\Rightarrow$ Stir with a bar} & \textbf{Action:}\emph{Make}\\
     & \textbf{Object:}\emph{Cocktail}\\
     \hline
     \multirow{2}{1.\linewidth}{\todo{Obtain a copy $\Rightarrow$ Look up unfamiliar words%$\Rightarrow$ Learn the story behind
     $\Rightarrow$ Read aloud a couple of times}} & \textbf{Action:}\emph{Memorise}\\
     & \textbf{Object:}\emph{Poem}\\
    \bottomrule
    \end{tabular}
    }
    \caption{Examples of multi-axis type inference for event processes.}
    \label{tbl:example}
    %\vspace{-1em}
\end{table}
